A Maturity Assessment Framework for Conversational AI Development Platforms

Conversational Artificial Intelligence (AI) systems have recently sky-rocketed in popularity and are now used in many applications, from car assistants to customer support. The development of conversational AI systems is supported by a large variety of software platforms, all with similar goals, but different focus points and functionalities. A systematic foundation for classifying conversational AI platforms is currently lacking. We propose a framework for assessing the maturity level of conversational AI development platforms. Our framework is based on a systematic literature review, in which we extracted common and distinguishing features of various open-source and commercial (or in-house) platforms. Inspired by language reference frameworks, we identify different maturity levels that a conversational AI development platform may exhibit in understanding and responding to user inputs. Our framework can guide organizations in selecting a conversational AI development platform according to their needs, as well as helping researchers and platform developers improving the maturity of their platforms.

==> classification.tex <==
\section{Classification}
https://arxiv.org/pdf/1606.02270.pdf - general knowledge about natural language comprehension on input text and how these text strings are processed. Showing a new way of comprehending text using neural models.

https://arxiv.org/pdf/1906.00500.pdf - research of how the generation of coherent and understandable sentences are made in dialog systems, and how to make the as humane as possible.

(Prediction During Natural Language Comprehension - available from chalmers lib) - research about how natural language predicts words and sentences for faster processing and smoother interaction between system and user.

https://arxiv.org/ftp/arxiv/papers/1801/1801.03604.pdf - general information regarding alexa and conversational ai, with focus on language and speech recognition and generation on chapter 5. Techniques used for comprehension and indistinguishably between a system and a human.

https://languagetestingasia.springeropen.com/track/pdf/10.1186/s40468-018-0069-0 - evaluation of the cefr framework.

https://search-proquest-com.proxy.lib.chalmers.se/docview/2084297501/fulltextPDF/8E9109AE0FE745E0PQ/1?accountid=10041 (Evaluating Visual Reasoning Through
Grounded Language Understanding - available from chalmers lib) - research regarding the systems ability to understand natural language and how this data is used.

https://www.aclweb.org/anthology/H93-1004 - how natural language data is trained and evaluated to achieve maximum results, what data is crucial for the performance of the algorithms.

https://arxiv.org/pdf/1809.08267.pdf - survey of existing neural approaches within conversational ai and how these differ.

https://www.aclweb.org/anthology/W17-5522 - evaluation of different conversational ai's NLU algorithms and services.
